TiGer: Self-Supervised Purification for Time-evolving Graphs

Time-evolving graphs, such as social and citation networks, often contain noise that distorts structural and temporal patterns, adversely affecting downstream tasks, such as node classification. Existing purification methods focus on static graphs, limiting their ability to account for critical temporal dependencies in dynamic graphs. In this work, we propose TiGer (Time-evolving Graph purifier), a self-supervised method explicitly designed for time-evolving graphs. TiGer assigns two different sub-scores to edges using (1) self-attention for capturing long-term contextual patterns shaped by both adjacent and distant past events of varying significance and (2) statistical distance measures for detecting inconsistency over a short-term period. These sub-scores are used to identify and filter out suspicious (i.e., noise-like) edges through an ensemble strategy, ensuring robustness without requiring noise labels. Our experiments on five real-world datasets show TiGer filters out noise with up to 10.2% higher accuracy and improves node classification performance by up to 5.3%, compared to state-of-the-art methods.

==> 021_related.tex <==
% \subsection{Graph Purification}
% \label{sec:prelim:purification}

\smallsection{Graph purification.}
\textit{Graph purification} is widely used as a pre-processing step for utilizing graph-structured data for various downstream tasks~\cite{luo2021learning,shen2024graph,spinelli2021fairdrop,xu2022ned,entezari2020all,wu2019adversarial}.
Depending on the approach used to compute purification scores (see Sec.~\ref{sec:prelim}), graph purification methods can be broadly categorized into two types: (1) local similarity-based, (2) global similarity-based.

\textit{Local similarity-based} use connectivity relationships (e.g., neighbors) between \textit{each node pair} to compute purification scores. 
Representative examples include the Jaccard Coefficient~\cite{sathre2022edge} and the Adamic-Adar Index~\cite{tian2020exploiting}.
\textit{Global similarirty-based} approaches use \textit{the whole graph topology}, i.e., the adjacency matrix.
For instance, Singular Value Decomposition (SVD)~\cite{entezari2020all} assumes a low-rank structure of the adjacency matrix, while Graph Diffusion~\cite{klicpera2019diffusion} uses matrix power series of the adjacency matrix.

Most existing graph purification approaches are designed for static graphs and unsuitable for time-evolving graphs. 
A recent method~\cite{lee2023time} applies graph diffusion while incorporating the results from previous timestamps through weighted summation.
However, this approach over-simplifies temporal dependencies, limiting its effectiveness.
To the best of our knowledge, no other graph purification methods have been explicitly designed for time-evolving graph scenarios.

\smallsection{Temporal Patterns.}
Temporal patterns are underlying patterns in time-evolving graphs.
%Various tasks [cite] in time-evolving graphs can be addressed by capturing these temporal patterns.
In time-evolving graphs, temporal patterns can be divided into long-term and short-term patterns.

Long-term patterns represent the temporal dependency across a long-term period (e.g., long-term trend).
For instance, in a coauthorship network, long-term collaborative trends can exist, such as continuously collaborating with members of a specific research group over a long-term period.
%In this case, long-term patterns can be gradually changed over time
Various Dynamic Graph Neural Networks (DGNNs) have been proposed by encoding dynamic node representations to capture long-term patterns.
To do this, many existing DGNNs~\cite{pareja2020evolvegcn,sankar2020dysat,tgn_icml_grl2020} employ RNN modules and self-attention~\cite{vaswani2017attention} to effectively model temporal dependencies for capturing long-term patterns.

Short-term patterns represent the temporal smoothness across a short-term period.
For instance, in a social network, most users exhibit consistent interaction behaviors, with minimal changes in the neighbors they interact with during a short-term period, demonstrating the smooth and gradual evolution of their interaction patterns.
%most users don't dramatically change the neighbors they interact with over a short-term period, demonstrating temporal smoothness in their interaction patterns. 
Notably, many studies~\cite{lee2024spear,lee2024slade,tian2021self,yu2017link,zhu2022dynamic} based on DGNNs incorporate short-term patterns, assuming that node representations evolve gradually over time without significant changes within a short-term period.



%Various tasks [cite] in time-evolving graphs can be addressed by capturing these temporal patterns.

%(12312312312313131)

%\begin{comment}
%\smallsection{Dynamic Graph Neural Networks (DGNNs).}
%\jongha{
%\textit{DGNNs} aim to capture temporal (spec., long-term and short-term) patterns of nodes in dynamic graphs by encoding their dynamic representations. Various DGNN models have been proposed to capture long-term patterns.}
%\textit{DGNNs} aim to capture the evolving temporal and structural patterns of nodes in dynamic graphs by encoding their dynamic representations.
%Various DGNN models have been proposed.
%EvolveGCN~\cite{pareja2020evolvegcn} uses an RNN module to evolve GCN~\cite{kipf2016semi} parameters over time, dynamically generating node representations.
%DySAT~\cite{sankar2020dysat} applies GAT~\cite{velivckovic2018graph} to each graph snapshot and uses self-attention~\cite{vaswani2017attention} along the temporal dimension.
%TGN~\cite{tgn_icml_grl2020} employs memory modules to construct dynamic node representations by capturing long-term patterns.
%TGAT~\cite{xu2020inductive} leverages temporal encodings and graph attention to incorporate high-resolution temporal information to construct dynamic node representations.
%Notably, many studies~\cite{lee2024spear,lee2024slade,tian2021self,yu2017link,zhu2022dynamic} consider \textit{temporal smoothness}, assuming that node representations evolve \textit{gradually} over time and avoiding preventing short-term structural drift.

%\jongha{
%Many studies consider temporal smoothness for modeling short-term patterns, assuming that node representations evolve \textit{gradually} over time and avoid preventing short-term structural drift.
%To do this, they generally utilize additional regularization terms for smoothness.}

%However, existing DGNNs face challenges when directly applied to graph purification in time-evolving graphs.
%Most DGNNs are trained using graph snapshots up to a specific time point.
%However, noise within these training snapshots can significantly hinder the training process. 
%Consequently, DGNNs may struggle to learn accurate structural and temporal patterns in the early stages of dynamic graphs, where limited training data is available, leading to a cold start problem.
%As a result, noisy edges that are not effectively filtered early persist in the training data, preventing DGNN models from learning correct patterns and causing the purification process to collapse.
%To address this, additional purification methods, such as proximity-based techniques or surrogate models, are needed to handle the cold start problem without relying on training.
%Additionally, since time-evolving graphs are a specific type of dynamic graphs (see Sec.~\ref{sec:prelim}), existing DGNNs designed for general dynamic graphs may not be sufficient. 
%Specialized techniques tailored for time-evolving graphs are needed to more effectively capture their temporally evolving structural patterns.
%\end{comment}

==> prev/03_limitations.tex <==
\begin{figure*}[t]
    \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/limit/lim1_school.pdf}
        \caption{\textsc{School}}
        \label{fig:limit:lim1_school}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/limit/lim1_brain.pdf}
        \caption{\textsc{Brain}}
        \label{fig:limit:lim1_brain}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/limit/lim1_patent.pdf}
        \caption{\textsc{Patent}}
        \label{fig:limit:lim1_patent}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/limit/lim1_dblp.pdf}
        \caption{\textsc{DBLP}}
        \label{fig:limit:lim1_dblp}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/limit/lim1_arXivAI.pdf}
        \caption{ArXivAI}
        \label{fig:limit:lim1_arXivAI}
    \end{subfigure} 
    \caption{
    aaaaa
    }
    \label{fig:limit:lim1}
\end{figure*}

\smallsection{Overview.} 
We observe that when existing graph filtering methods are applied temporally (i.e., performing filtering at each timestep), they exhibit several limitations.

\begin{enumerate}[leftmargin=2.5em,topsep=0pt]
    \item[\textbf{L1)}] \textbf{Short-sighted Filtering (Fig.~\ref{fig:limit:lim1})}: 
    Temporal graph filtering easily becomes suboptimal. Since temporal graphs accumulate information over time, applying simple rule-based filtering methods at each moment is not well-suited to this dynamic context.
    
    \item[\textbf{L2)}] \textbf{Excessive Filtering (Fig.~\ref{fig:lim:lim2})}: 
    Temporal graph filtering can lead \textit{temporally corrected nodes} (Definition~\ref{defn:temp}) to incorrect predictions.
\end{enumerate}

\subsection{Limitation 1: Short-sighted Filtering} Temporal graph filtering easily becomes suboptimal. Since temporal graphs accumulate information over time, applying simple rule-based filtering methods at each moment is not well-suited to this dynamic context.

    
\subsection{Limitation 2: Excessive Filtering}
Temporal graph filtering can lead \textit{temporally corrected nodes} (Definition~\ref{defn:temp}) to incorrect predictions.


\begin{defn}[Temporally corrected node]
\label{defn:temp}
Let $V^{c}$ denote the set of temporally corrected nodes. 
A node $v \in V^{c}$ is defined as one that:
(1) First appears at timestep $t$ and is initially misclassified by GNN, i.e., $f_{\theta}^{t}(v) \neq y_{t}(v)$,
(2) is eventually correctly classified at the final timestep $T$, where $f_{\theta}^{T}(v) = y_{t}(v)$.
\end{defn}




